Non-negative DAG Learning from Time-Series Data

This work aims to learn the directed acyclic graph (DAG) that captures the instantaneous dependencies underlying a multivariate time series. The observed data follow a linear structural vector autoregressive model (SVARM) with both instantaneous and time-lagged dependencies, where the instantaneous structure is modeled by a DAG to reflect potential causal relationships. While recent continuous relaxation approaches impose acyclicity through smooth constraint functions involving powers of the adjacency matrix, they lead to non-convex optimization problems that are challenging to solve. In contrast, we assume that the underlying DAG has only non-negative edge weights, and leverage this additional structure to impose acyclicity via a convex constraint. This enables us to cast the problem of non-negative DAG recovery from multivariate time-series data as a convex optimization problem in abstract form, which we solve using the method of multipliers. Crucially, the convex formulation guarantees global optimality of the solution. Finally, we assess the performance of the proposed method on synthetic time-series data, where it outperforms existing alternatives.

==> figs/all_exps.tex <==
\begin{tikzpicture}
    % ======================================
    % 1. CARGA DE DATOS (Todos los paneles)
    % ======================================
    
    % --- PANEL A: SAMPLES (W y A) ---
    \pgfplotstableread[col sep=comma]{data/samples/samples_errW_med.csv}\sampWmed
    \pgfplotstableread[col sep=comma]{data/samples/samples_errW_prctile25.csv}\sampWlow
    \pgfplotstableread[col sep=comma]{data/samples/samples_errW_prctile75.csv}\sampWhigh
    \pgfplotstableread[col sep=comma]{data/samples/samples_errA_med.csv}\sampAmed
    \pgfplotstableread[col sep=comma]{data/samples/samples_errA_prctile25.csv}\sampAlow
    \pgfplotstableread[col sep=comma]{data/samples/samples_errA_prctile75.csv}\sampAhigh

    % --- PANEL B: NODES (Datos F1-Score) ---
    % Nota: He verificado que uses 'nodes_fsW' como en tu último snippet
    \pgfplotstableread[col sep=comma]{data/nodes/nodes_fsW_med.csv}\nodeWmed
    \pgfplotstableread[col sep=comma]{data/nodes/nodes_fsW_prctile25.csv}\nodeWlow
    \pgfplotstableread[col sep=comma]{data/nodes/nodes_fsW_prctile75.csv}\nodeWhigh
    \pgfplotstableread[col sep=comma]{data/nodes/nodes_fsA_med.csv}\nodeAmed
    \pgfplotstableread[col sep=comma]{data/nodes/nodes_fsA_prctile25.csv}\nodeAlow
    \pgfplotstableread[col sep=comma]{data/nodes/nodes_fsA_prctile75.csv}\nodeAhigh

    % --- PANEL C: LAGS (Datos NFE) ---
    \pgfplotstableread[col sep=comma]{data/lags/lags_errW_med.csv}\lagsWmed
    \pgfplotstableread[col sep=comma]{data/lags/lags_errW_prctile25.csv}\lagsWlow
    \pgfplotstableread[col sep=comma]{data/lags/lags_errW_prctile75.csv}\lagsWhigh
    \pgfplotstableread[col sep=comma]{data/lags/lags_errA_med.csv}\lagsAmed
    \pgfplotstableread[col sep=comma]{data/lags/lags_errA_prctile25.csv}\lagsAlow
    \pgfplotstableread[col sep=comma]{data/lags/lags_errA_prctile75.csv}\lagsAhigh

    % Configuración común
    \pgfmathsetmacro{\opacity}{0.2} 

    % ======================================
    % 2. CONFIGURACIÓN DEL GROUPPLOT
    % ======================================
    \begin{groupplot}[
        group style={
            group size=3 by 1,        % 3 columnas, 1 fila
            horizontal sep=1.3cm,     % Separación entre gráficas
            vertical sep=0cm,
        },
        width=0.33\textwidth,         % Ancho individual
        height=5cm,                   % Altura uniforme
        grid style={gray!30},
        grid=major,
        tick label style={font=\footnotesize},
        label style={font=\footnotesize},
    ]

    % ---------------------------------------------------------
    % PANEL (a): Samples (Log-Log) - NFE
    % ---------------------------------------------------------
    \nextgroupplot[
        xmode=log, ymode=log,
        % IMPORTANTE: Doble llave {{...}} para proteger el paréntesis (a)
        xlabel={{Number of samples $T$}}, 
        ylabel={NFE},
        xmin=90, xmax=5500,
        xtick={100, 1000, 5000},
        xticklabels={$10^2$, $10^3$, $5{\times}10^3$},
        ymin=1e-3, ymax=2,
    ]
        % --- CVX (Blue) ---
        \addplot [name path=sWtop, draw=none, forget plot] table [x=xaxis, y=Adam] \sampWhigh;
        \addplot [name path=sWbot, draw=none, forget plot] table [x=xaxis, y=Adam] \sampWlow;
        \addplot [blue!50, opacity=\opacity, forget plot] fill between[of=sWtop and sWbot];
        \addplot [blue, thick, mark=*, mark options={scale=0.6}] table [x=xaxis, y=Adam] {\sampWmed};

        \addplot [name path=sAtop, draw=none, forget plot] table [x=xaxis, y=Adam] \sampAhigh;
        \addplot [name path=sAbot, draw=none, forget plot] table [x=xaxis, y=Adam] \sampAlow;
        \addplot [blue!50, opacity=\opacity, forget plot] fill between[of=sAtop and sAbot];
        \addplot [blue, thick, dashed, mark=*, mark options={solid, scale=0.6}] table [x=xaxis, y=Adam] {\sampAmed};

        % --- DYNO (Red) ---
        \addplot [name path=dWtop, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \sampWhigh;
        \addplot [name path=dWbot, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \sampWlow;
        \addplot [red!50, opacity=\opacity, forget plot] fill between[of=dWtop and dWbot];
        \addplot [red!90!black, thick, mark=x, mark options={scale=0.8}] table [x=xaxis, y=DYNOTEARS] {\sampWmed};

        \addplot [name path=dAtop, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \sampAhigh;
        \addplot [name path=dAbot, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \sampAlow;
        \addplot [red!50, opacity=\opacity, forget plot] fill between[of=dAtop and dAbot];
        \addplot [red!90!black, thick, dashed, mark=x, mark options={solid, scale=0.8}] table [x=xaxis, y=DYNOTEARS] {\sampAmed};

    % ---------------------------------------------------------
    % PANEL (b): Nodes (Semilog-X) - F1 Score
    % ---------------------------------------------------------
    \nextgroupplot[
        xmode=log, ymode=normal,
        % IMPORTANTE: Doble llave {{...}}
        xlabel={{Number of nodedasdadss $N$}},
        ylabel={F1-score},
        xmin=25, xmax=1000,
        xtick={25, 100, 1000},
        xticklabels={25, 100, 1000},
        ymin=0.74, ymax=1.01,
        % LEYENDA GLOBAL
        legend columns=4,
        legend style={
            at={(0.5, 1.15)},
            anchor=south,
            draw=black,
            /tikz/every even column/.append style={column sep=0.3cm}
        }
    ]
        % --- CVX (Blue) ---
        \addplot [name path=nWtop, draw=none, forget plot] table [x=xaxis, y=Adam] \nodeWhigh;
        \addplot [name path=nWbot, draw=none, forget plot] table [x=xaxis, y=Adam] \nodeWlow;
        \addplot [blue!50, opacity=\opacity, forget plot] fill between[of=nWtop and nWbot];
        \addplot [blue, thick, mark=*, mark options={scale=0.6}] table [x=xaxis, y=Adam] {\nodeWmed};
        \addlegendentry{CVX-DYN ($\hbW$)} 

        \addplot [name path=nAtop, draw=none, forget plot] table [x=xaxis, y=Adam] \nodeAhigh;
        \addplot [name path=nAbot, draw=none, forget plot] table [x=xaxis, y=Adam] \nodeAlow;
        \addplot [blue!50, opacity=\opacity, forget plot] fill between[of=nAtop and nAbot];
        \addplot [blue, thick, dashed, mark=*, mark options={solid, scale=0.6}] table [x=xaxis, y=Adam] {\nodeAmed};
        \addlegendentry{CVX-DYN ($\hbA$)} 

        % --- DYNO (Red) ---
        \addplot [name path=dnWtop, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \nodeWhigh;
        \addplot [name path=dnWbot, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \nodeWlow;
        \addplot [red!50, opacity=\opacity, forget plot] fill between[of=dnWtop and dnWbot];
        \addplot [red!90!black, thick, mark=x, mark options={scale=0.8}] table [x=xaxis, y=DYNOTEARS] {\nodeWmed};
        \addlegendentry{DYNO ($\hbW$)} 

        \addplot [name path=dnAtop, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \nodeAhigh;
        \addplot [name path=dnAbot, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \nodeAlow;
        \addplot [red!50, opacity=\opacity, forget plot] fill between[of=dnAtop and dnAbot];
        \addplot [red!90!black, thick, dashed, mark=x, mark options={solid, scale=0.8}] table [x=xaxis, y=DYNOTEARS] {\nodeAmed};
        \addlegendentry{DYNO ($\hbA$)} 

    % ---------------------------------------------------------
    % PANEL (c): Lags (Semilog-Y) - NFE
    % ---------------------------------------------------------
    \nextgroupplot[
        xmode=normal, ymode=log,
        % IMPORTANTE: Doble llave {{...}}
        xlabel={{Number of lags $P$}},
        ylabel={NFE},
        xmin=1, xmax=4,
        xtick={1,2,3,4},
        ymin=1e-3, ymax=0.2,
    ]
        % --- CVX (Blue) ---
        \addplot [name path=lWtop, draw=none, forget plot] table [x=xaxis, y=Adam] \lagsWhigh;
        \addplot [name path=lWbot, draw=none, forget plot] table [x=xaxis, y=Adam] \lagsWlow;
        \addplot [blue!50, opacity=\opacity, forget plot] fill between[of=lWtop and lWbot];
        \addplot [blue, thick, mark=*, mark options={scale=0.6}] table [x=xaxis, y=Adam] {\lagsWmed};

        \addplot [name path=lAtop, draw=none, forget plot] table [x=xaxis, y=Adam] \lagsAhigh;
        \addplot [name path=lAbot, draw=none, forget plot] table [x=xaxis, y=Adam] \lagsAlow;
        \addplot [blue!50, opacity=\opacity, forget plot] fill between[of=lAtop and lAbot];
        \addplot [blue, thick, dashed, mark=*, mark options={solid, scale=0.6}] table [x=xaxis, y=Adam] {\lagsAmed};

        % --- DYNO (Red) ---
        \addplot [name path=dlWtop, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \lagsWhigh;
        \addplot [name path=dlWbot, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \lagsWlow;
        \addplot [red!50, opacity=\opacity, forget plot] fill between[of=dlWtop and dlWbot];
        \addplot [red!90!black, thick, mark=x, mark options={scale=0.8}] table [x=xaxis, y=DYNOTEARS] {\lagsWmed};

        \addplot [name path=dlAtop, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \lagsAhigh;
        \addplot [name path=dlAbot, draw=none, forget plot] table [x=xaxis, y=DYNOTEARS] \lagsAlow;
        \addplot [red!50, opacity=\opacity, forget plot] fill between[of=dlAtop and dlAbot];
        \addplot [red!90!black, thick, dashed, mark=x, mark options={solid, scale=0.8}] table [x=xaxis, y=DYNOTEARS] {\lagsAmed};

    \end{groupplot}
\end{tikzpicture}
